LLM-Powered Code Vulnerability Repair with Reinforcement Learning and Semantic Reward

In software development, the predominant emphasis on functionality often supersedes security concerns, a trend gaining momentum with AI-driven automation tools like GitHub Copilot. These tools significantly improve developers' efficiency in functional code development. Nevertheless, it remains a notable concern that such tools are also responsible for creating insecure code, predominantly because of pre-training on publicly available repositories with vulnerable code. Moreover, developers are called the "weakest link in the chain" since they have very minimal knowledge of code security. Although existing solutions provide a reasonable solution to vulnerable code, they must adequately describe and educate the developers on code security to ensure that the security issues are not repeated. Therefore we introduce a multipurpose code vulnerability analysis system \texttt{SecRepair}, powered by a large language model, CodeGen2 assisting the developer in identifying and generating fixed code along with a complete description of the vulnerability with a code comment. Our innovative methodology uses a reinforcement learning paradigm to generate code comments augmented by a semantic reward mechanism. Inspired by how humans fix code issues, we propose an instruction-based dataset suitable for vulnerability analysis with LLMs. We further identify zero-day and N-day vulnerabilities in 6 Open Source IoT Operating Systems on GitHub. Our findings underscore that incorporating reinforcement learning coupled with semantic reward augments our model's performance, thereby fortifying its capacity to address code vulnerabilities with improved efficacy.

==> sections/2_problem.tex <==
\subsection{Threat Model}

In the context of implementing LLMs for vulnerability analysis for research on cybersecurity, we explored our threat model in-depth, encompassing two critical types of threat actors. The first type involves LLMs and open-source solutions, serving as a helping tool for developers to find or generate code snippets based on various issues or instructions. Although the LLM-generated code is not intentionally malicious, it exhibits a bias towards producing code with potential vulnerabilities due to the lack of training on generating secure code. Additionally, developers often rely on code snippets from open-source solutions like GitHub and StackOverflow, introducing the risk of code reuse or obfuscation which may further propagate vulnerabilities.

The second group of actors consists of developers who may need adequate training or awareness of code security and its potential privacy implications. Such developers pose a risk to their projects by using slightly modified versions of code generated by LLMs or sourced from open repositories without conducting thorough verification. This practice leaves the entire software application vulnerable to potential threats and exploits. Our research focuses on addressing these concerns and proposing solutions to enhance code security practices and mitigate risks in the software development process.

Our threat model mainly focuses on code-based vulnerabilities produced by code obfuscation at the function level of a program. We support analyzing vulnerabilities in code development for beginner programmers for simple tasks and complicated tasks for experienced developers. Our focused vulnerabilities are twofold. First, these vulnerabilities crash the program by causing memory leaks or buffer overflows. Secondly, we also focus on the vulnerabilities that do not crash the program but let threat actors take control of a system by code or malware injection by metamorphosis, illegal memory access, and taking root access to a system.

We divided our working procedure into three steps in our approach to solving and aiding developers with code security knowledge. Firstly, we help the developers identify vulnerable code. Then we suggest developers with a possible fix for the vulnerable code using an LLM-based generative model. Furthermore, since the developers are less trained in security, we provide a detailed description of the vulnerability of the code with a customized code-specific description explaining why the code is vulnerable and a possible hint to solving the code.

%\red{Motivation with examples: Real world something bad about this. Attack on IoT OS}


\subsection{Motivation}
\label{sec:motivation}
With the advent of OSS \cite{kim2017vuddy} and LLM-based code development \cite{murali2023codecompose}, vulnerabilities emerging due to code obfuscation procedures have become a major challenge. Developers use LLM and OSS generated to modify these according to the need of their applications. Therefore, if the original code was vulnerable, code obfuscation by the developers could rapidly spread the vulnerable code. Although various works are done on code clone detection \cite{woo2022movery} \cite{kim2017vuddy}, our goal is to analyze the quality of the SOTA works vulnerability detection model on obfuscated code.



\begin{table}[t]
\caption{This table demonstrates how the SOTA models perform poorly on vulnerability identification from IoT Operating Systems with obfuscated code.}
\label{tab:tab1}
\centering
\begin{tabular}{@{}l|c|c@{}}
\toprule
\textbf{Model} & \multicolumn{1}{c|}{\textbf{Dataset}}                                                     & \textbf{Correct Prediction} \\ \midrule
VulDeelocator \cite{li2018vuldeepecker}   & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}100 Sample Code\\ from IoT \\ Device OS\end{tabular}} & 45                          \\
Devign \cite{li2021vuldeelocator}  &                                                                                     & 61           \\
VELVET \cite{zhou2019devign}         &                                                                                                  & 64                          \\
PFGCN \cite{ding2021velvet}         &                                                                                                  & 67                          \\
                         \bottomrule
\end{tabular}
\end{table}





To evaluate the effectiveness of current SOTA models, we curated a small dataset comprising 100 examples extracted from IoT operating systems, encompassing both vulnerable and non-vulnerable instances. Notably, we ensured that this dataset did not overlap with the training data used for the model. We intentionally modified these through code obfuscation techniques, such as dead code insertion, code reformatting, and variable and function renaming. The examples retained their original functionality post-compilation. This simulation was a rigid test of the model's capacity to detect developer-initiated code modifications/obfuscations from open-source solutions and LLMs while preserving core functionality.

Table \ref{tab:tab1} presents compelling results from the experiment, illustrating the model's performance on the 100 examples. VulDeelocator \cite{li2021vuldeelocator} demonstrated subpar performance, identifying only 45 vulnerable code instances, while PFGCN \cite{islam2023unbiased} showed relatively better performance by capturing 67 vulnerable code instances. These findings underline the limitations of existing models, rendering them less dependable for real-world scenarios where developers require more reliable and accurate vulnerability detection.




\subsection{Problem Formulation}

\paragraph{\textbf{Vulnerability Repair and Description}}
Our proposed system leverages a Large Language Model-based reinforcement learning through human feedback (RLHF) approach that incorporates learning from training data and human feedback. Our methodology employs an RLHF on top of an LLM to repair and describe vulnerabilities generated from source code. We use function as the granular input to the LLM. 

We define each vulnerable function $f_{vul}$ and the repaired function as $f_{rep}$. We denote the vulnerability description as $D$. We tokenize the vulnerable function $f_{vul}$ and convert it to tokens $T$. Each token $t_i \in T$ is converted to an embedding $e_i \in E_{mbd}$


Our methodology employs a multitask function that undertakes vulnerability identification, repair, and description. Initially, it ascertains identifications of the vulnerable code $V$, then the repair of the vulnerability $f_{rep}$, and then provides a description $D$ of the vulnerability. Let us consider our vulnerability multitask function $v_m$ that maps the token embeddings to repaired code $f_{rep}$ and vulnerability description $D$.

%category, CWE denoted as $CWE$, that a vulnerable input function $p_i$ aligns with. If a vulnerability is detected within $p_i$, the model further localizes the vulnerable tokens, designating this set as the vulnerability localization range, $Vul_{Code}[T_{start}, T_{end}]$. In the context of our model, we define three outputs: the vulnerability classification CWE, the vulnerability localization $Vul_{Code}$, and the vulnerability description $D_{escription}$. We utilize our ensemble function $f(h)$ as a multitasking tool that maps the graph structure $\mathcal{G}_{raph}$ and the embeddings $E_{mbeddings}$ to these outputs.

\begin{equation}
\label{eqn:1}
v_m(E_{mbd}) = V
\end{equation}

\begin{equation}
\label{eqn:2}
v_m(E_{mbd}) = f_{rep}
\end{equation}

\begin{equation}
\label{eqn:3}
v_m(E_{mbd}) = D
\end{equation}


We task our LLM for vulnerability identification and generate the vulnerability repair and description.

\paragraph{\textbf{Reinforcement Learning from Human Feedback}}

The goal of using reinforcement learning through human feedback is to ensure the model's descriptions are verified by a human agent or developer during the training process. After initial training, we consider the developer interacting with the outcome of the LLM over the custom description task. Unlike a regular RL technique, we provide feedback to the model after each outcome by a human agent in the form of positive or negative reinforcement. This outcome or reward is used as a loss value to fine-tuning the LLM.

Given a code and two descriptions, one from model and another from ground truth, are judged by humans. The judgment is in the form of a reward $r_\theta$ from human labels. Then the reward fine-tunes the LLM. We train this model to predict a better description $D \in D^1, D^2$ for a vulnerable function $f_{vul}$. If the description preferred by the human is $D^i$, the loss for reward model can be written as:

\begin{equation}
    \label{eqn:3}
    L(r_\theta) = E_{D^1 D^2} [log (\sigma(r_\theta (f_{vul}, D^1) - r_\theta (f_{vul}, D^2) )]
\end{equation}

where $r_\theta (f_{vul}, D^i_{esc})$ is the scalar output of the reward model for vulnerable function $f_{vul}$ and description $D^i_{esc}$ and $\theta$ is the learnable parameter.


In this study, we aim to address three research questions (RQs) concerning the effectiveness and capabilities of our proposed system, DevSecLLM, for vulnerability analysis and code repair in potentially vulnerable obfuscated code developed by human developers:

\begin{itemize}
    \item \textbf{RQ1:} Can our proposed system effectively identify vulnerabilities in obfuscated code developed by human developers? 
 
    \item \textbf{RQ2:} Does our system demonstrate accurate and reliable code repair capabilities?
  
    \item \textbf{RQ3:} Can our model generate customized code-specific cybersecurity descriptions of the vulnerable code to aid developers in validating the repaired code?
    


\end{itemize}

Through experimentation and analysis, we aim to provide valuable insights into the efficacy of our proposed system and its potential to enhance code security practices in obfuscated code development. By addressing these research questions, we aim to contribute to advancing cybersecurity techniques for mitigating vulnerabilities in code developed by human programmers.



==> sections/backup.tex <==

%To answer this question, we analyzed in-depth how developers interact with code generation models like Code Inspector, Codex, GitHub Copilot, etc. GitHub Copilot is one of the most popular AI-powered tools professionals, and students use in software development. We consider the impact of developing code using AI in two stages. One is by students, and the other one is by professional developers. Therefore we produce different instructions for each category. We consider zero-day vulnerability as the vulnerable code generated by AI-powered tools.

%For the student category, we followed the work by Puryear et al.\cite{puryear2022github} to generate different prompts related to students. These relate to functions and code, including function, loop, arithmetic, and API calls. Also, we included data-related data structure and algorithm-related tasks like binary search, linked list generation, graph search algorithms, etc. We picked more challenging items related to software development tasks for the professional developer category. These tasks are, as suggested by CodeCompose \cite{murali2023codecompose}, mostly about executing some operation based on some logic, generating error messages, or optimizing the program for faster runtime. 

%We generated a small dataset with a specific set of questions for software developers and software development professionals. Table \ref{tab} shows a summarized version of the category of questions we ask to the AI-based tools and captures their response. In order to conduct this experiment, we used different AI tools like Codex, PolyCoder, and GitHub Copilot and generated five responses for each problem. We analyzed each type of tool individually, and our security experts the responses from the tools manually. If the answer is satisfactory to the security expert, we consider it a "good outcome"; otherwise, we consider it a "bad outcome".

%The expected output from our model is the repaired code with a customized vulnerability description. Our analysis shows that, among these three tools, \color{red} X and Y generated the minimum number of errors for the student category. On the other hand, Z and X produce better performance for software development-related tasks. This infers that X and Y generate fewer vulnerabilities. \color{black} This analysis also shows that our model can repair and describe vulnerabilities it has never seen before. We are concluding that students and professional software developers could use our system reliably.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Users}                                                                           & \textbf{Question} & \textbf{Total} & \textbf{Correct} & \textbf{Incorrect} \\ \midrule
\multirow{3}{*}{\textbf{Students}}                                                       & Binary Search     & 5              &                  &                    \\
   & Linked List       & 8              &                  &                    \\
   & Graph Algorithms  & 4              &                  &                    \\ \midrule
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Software \\ Developers\end{tabular}}} & Logic Execution   & 9              &                  & \\
    & Error Message     & 3              &                  &                    \\
    & Optimize          & 6              &                  &              \\
    \bottomrule
\end{tabular}
\end{table}


%%%%%%%% Table 1   %%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\caption{BLEU and Rouge-L score on our dataset with models trained on code. We use LLMs with multiple parameters to compare our work.}
\label{tab:tab1}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Dataset}                       & \textbf{Model}             & \textbf{Parameter} & \textbf{CodeBLEU} & \textbf{Rouge-L} \\ \midrule
\multirow{7}{*}{\textbf{Our Dataset}} & \multirow{1}{*}{StarCoder} & 1.1B                  &        0.17           &       0.13           \\
        &                  \\ \cmidrule(l){2-5} 
    &                            & 1B                 &                   &         \\
    
    & Codegen2-Multi             & 1B                 &     0.42          &  0.31\\
    &                            & 3.7B               &     0.74          & 0.96               \\ \cmidrule(l){2-5} 
    & CodeGen-Multi                     & 2B                &     0.80              &   0.98               \\
    &                            & 6.7                &      0.82             &   0.98               \\ \cmidrule(l){2-5} 
    & Ours                       & 7B                 & 0.5471           & 0.5718           \\ \midrule
    &                            &                    &                   &         \\
    &                            &                    &                   &        \\ %\bottomrule
\end{tabular}

\end{table}



%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\centering
\label{tab:motivation}
\caption{This is a caption}
\begin{tabular}{@{}llcl@{}}
\toprule
\textbf{Model}  & \textbf{Parameters} & \multicolumn{1}{l}{\textbf{Total Examples}} & \textbf{Correct Pred.} \\ \midrule
T5              & 770M                & \multirow{5}{*}{100}                        & 57                           \\
CodeT5          & 770M                &                                             & 61                           \\
Codegen2        & 1B                  &                                             & 64                           \\
Codegen2        & 3.7B                &                                             & 71                           \\
CodeGen2 (Ours) & 7B                  &                                             & \textbf{74}                  \\ \bottomrule
\end{tabular}
\end{table}




%%%%%%%%%  CVE Fixes and BigVul %%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[b]
\caption{BLEU and Rouge-L score on Big-Vul and CVEfixes Dataset}
\label{tab:tab2}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Dataset}                       & \textbf{Model}             & \textbf{Parameter} & \textbf{CodeBLEU} & \textbf{Rouge-L} \\ \midrule

\multirow{11}{*}{\textbf{Big-Vul}} & \multirow{3}{*}{StarCoder} & 1B                 &                   &                  \\
                                       &                            & 3.7B               &                   &                  \\
                                       &                            & 7B                 &                   &                  \\ \cmidrule(l){2-5} 
                                       &                            & 1B                 &                   &                  \\
                                       & CodeT5               & 3.7B               &                   &                  \\
                                       &                            & 7B                 &                   &                  \\ \cmidrule(l){2-5} 
                                       & Codegen2-Multi             & 1B                 &                   &                  \\
                                       &                            & 7B                 &                   &                  \\ \cmidrule(l){2-5} 
                                       & CodeGen                     & 3.7                &                   &                  \\
                                       &                            & 6B                &        0.82           &    0.98              \\ \cmidrule(l){2-5} 
                                       & Ours                       & 7B                 & 0.5471           & 0.5718           \\ \midrule

                                       
                                    \textbf{CVEFixes}   &                            &                    &                   &                  \\
                                       &                            &                    &                   &                  \\ 
                                       

                                       \bottomrule


\end{tabular}

\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[b]
\caption{RLHF Comparison}
\label{tab:tab3}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Dataset}                       & \textbf{Model}             & \textbf{Parameter} & \textbf{CodeBLEU} & \textbf{Rouge-L} \\ \midrule

\multirow{6}{*}{\textbf{Dataset}} & \multirow{3}{*}{CodeGen2} & 1B                 &          0.51         &      0.87            \\
                                       &                            & 3.7B               &     0.72              &        0.98          \\
                                       &                            & 7B                 &       0.45            &     0.70             \\ \cmidrule(l){2-5} 
                                       &                            & 1B                 &                   &                  \\
                                       & Codegen2 (RLHF)               & 3.7B               &                   &                  \\
                                       &                            & 7B                 &                   &                  \\ 
                                       

                                       \bottomrule
\end{tabular}

\end{table}



%%%%%%%%%%%%   Introduction Last Day of Submission  %%%%%%%%%%%%%



Cybersecurity and code vulnerabilities constitute significant concerns in our digital age \cite{executiveorder, jointadvisory}. Addressing these issues is crucial given that such vulnerabilities represent weaknesses and security gaps that cybercriminals could exploit to carry out malicious activities \cite{cisaalerts}. Vulnerabilities can arise due to a variety of reasons, including technical glitches, human error, or even propagation via third-party Open-Source Software (OSS) reuse \cite{woo2022movery, jang2012redebug, kim2017vuddy}.

% which could lead to serious repercussions like data breaches \cite{}, identity theft \cite{}, and financial losses \cite{weconomicforum, deloitte}.


For instance, the Null Pointer Exception, often referred to as the \textit{Billion Dollar Mistake} \cite{eichholz2019avoid}, is one of the most prevalent programming flaws and vulnerabilities that allow malware and viruses to propagate. While this exception can be fixed by inserting a conditional statement, it still ranks among the top 25 Common Weakness Enumeration (CWE) vulnerabilities published by MITRE in 2022 \cite{cwe}. According to an article published by Cybersecurity Ventures \cite{venture}, the estimated annual cost ofcybercrime is predicted to skyrocket to a staggering 10.5 trillion dollars by 2025. Additionally, a report from the World Economic Forum \cite{wef} reveals that merely 4\% of the security experts are confident in the security measures implemented for Internet-connected devices. These alarming statistics and the current fragile state of OSS security highlight the significant challenge of establishing robust software security. Moreover, it emphasizes the crucial role of researchers and software developers in devising effective techniques and strategies to address code vulnerabilities. Failure to effectively address these risks can lead to substantial financial losses, irreparable damage to organizational reputations, and eroding public trust.



% \red{LLM and open source based Software Development}
\textbf{Code Autocompletion Advancements.} In recent years, significant advancements in neural language modeling have led to impressive enhancements in code autocompletion, a crucial feature in modern code editors and Integrated Development Environments (IDEs). Utilizing state-of-the-art Large Language Model (LLM)-based auto-completion tools, such as \texttt{GitHub Copilot} \cite{copilot}, can remarkably boost a developer's productivity by offering context-driven suggestions of statements or tokens \cite{chen2021evaluating}. Comparative evaluations have demonstrated that alternative code autocompletion solutions, including \texttt{TabNine} \cite{tabnine} and \texttt{IntelliCode} \cite{intellij}, exhibit superior performance compared to autocomplete tools reliant on static analysis. Moreover, the effectiveness of LLMs has been amplified with the introduction of open-source applications including \texttt{ChatGPT}, \texttt{GitHub Copilot} which are proving valuable in various areas including, software architecture \cite{ahmad2023towards} and software development \cite{murali2023codecompose} \cite{ross2023programmer}. 





% \textbf{Code Reuse Trends and Security Concerns in Software Development.} Notably, code reuse has become a habitual trend and an acceptable form of software development \cite{verdi2020empirical}. Nevertheless, code from OSS solutions comes with intentional and unintentional security vulnerabilities or weaknesses \cite{zhang2021study} \cite{verdi2020empirical}. Not to mention, the absence of transparency when considering newly-surfaced LLM-based code autocompletion tools that are mostly pre-trained and fine-tuned on unsecured and openly accessible repositories such as \texttt{GitHub} \cite{chen2021evaluating}. By adapting to this trend, software developers are continuously reusing codes from OSS solutions and/or LLM-based code autocompletion tools while applying code cloning \cite{huang2023our} or structurally changing \cite{ragkhitwetsagul2019toxic} with or without interfering with the main code functionality. As a result, outstanding concerns may arise, namely; \textit{\textbf{(i)}} \textit{inherited security code vulnerabilities from OSS solutions}, leading to vulnerability spreading \cite{sharif2008impeding, o2011obfuscation} in the form of modified (metamorphic) code \cite{borello2008code} and making it exponentially harder for antivirus products to detect malware especially in Linux-based environments \cite{de2021mmale} and Internet of Things (IoT)-related Operating Systems (OS) \cite{ravi2022static}; and \textit{\textbf{(ii)}} \textit{generated security code vulnerabilities from LLM-based code autocompletion tools}, manipulated by adding specially-crafted code to the training corpus during fine-tuning \cite{asare2022github, chen2021evaluating} and adversely influencing suggestions for attacker-chosen contexts \cite{schuster2021you} particularly in \texttt{ChatGPT} where it was found that 16 out of 21 security-related coding sessions are insecure while the rest could be improved with further prompting \cite{khoury2023secure} .
% To this end, the chaotic OSS solutions reuse coupled with the uncontrollable LLM-based code autocompletion tools impairs their effectiveness and results in critical security code vulnerabilities when applied to real-world tasks \cite{wu2022ai}.

\textbf{Code Reuse Trends and Security Concerns in Software Development.} Code reuse has become a pervasive practice in software development that has been earning wide acceptance \cite{verdi2020empirical}. However, it is important to acknowledge that code sourced from OSS solutions can harbor both intentional and unintentional security vulnerabilities \cite{zhang2021study, verdi2020empirical}. Equally important is the lack of transparency of newly-emerged developed code autocompletion tools based on LLMs. These tools, typically pre-trained and fine-tuned using code repositories that are insecure and publicly accessible (e.g., \texttt{GitHub}) \cite{chen2021evaluating}, can be influenced in a detrimental manner, particularly in situations involving attacker-chosen contexts \cite{schuster2021you}.

As developers adopt this trend, they frequently reuse code from OSS solutions and LLM-based code autocompletion tools. Sometimes, they resort to code cloning \cite{huang2023our} and/or perform structural modifications \cite{ragkhitwetsagul2019toxic} with or without affecting the main code functionality. This leads to significant concerns, namely; \textit{\textbf{(i)}} \textit{inherited security vulnerabilities from OSS solutions}, which lead to vulnerability propagation \cite{sharif2008impeding, o2011obfuscation} in the form of modified code \cite{borello2008code}; and \textit{\textbf{(ii)}} \textit{generated security vulnerabilities from LLM-based code autocompletion tools}, resulting in vulnerability propagation in the form of obfuscated code. As a result, the lack of control over LLM-based code autocompletion tools and the unregulated reuse of OSS solutions have extensive ramifications. This not only impairs their efficacy but also 
leads to critical security code vulnerabilities emerging when these solutions and tools are applied to real-world tasks \cite{wu2022ai}. In addition, one significant issue is the exponential difficulty faced by cybersecurity researchers and contemporary antivirus products in keeping track of the various vulnerability variants and their potential exploitation. This challenge becomes especially prominent in Linux-based environments \cite{de2021mmale} and Operating Systems (OS) related to the Internet of Things (IoT) \cite{ravi2022static}.


% manipulated by adding specially-crafted code to the training corpus during fine-tuning \cite{asare2022github, chen2021evaluating} and adversely influencing suggestions for attacker-chosen contexts \cite{schuster2021you} particularly in \texttt{ChatGPT} where it was found that 16 out of 21 security-related coding sessions are insecure while the rest could be improved with further prompting \cite{khoury2023secure} .









% \red{LLm plugged in everything. llm to generate code, devs use social network giThub, stack overflow.. use this case as well}

% \red{In many cases, vulnerabilities are introduced by software developers using code snippets from open-source solutions, such as Stack Overflow and GitHub.}

% \red{Vulnerability (use the term programmer) associated with AI assisted code}

% However, LLM-based code autocompletion tools are mostly pre-trained and fine-tuned on publicly available repositories from GitHub \cite{chen2021evaluating}. Moreover, the outcome of these models can be manipulated by adding specially-crafted code to the training corpus during fine-tuning, which can influence its suggestions for attacker-chosen contexts \cite{schuster2021you}. Studies by \cite{asare2022github} and \cite{chen2021evaluating} suggest that LLMs generate vulnerable code because similar examples were seen during training. A recent study \cite{khoury2023secure} on the performance of ChatGPT in generating source code found that out of 21 security-related coding sessions, 16 were insecure code, and only 7 cases could be improved with further prompting. Furthermore, code reuse has become an acceptable form of software development \cite{verdi2020empirical}. Nevertheless, code from crowd-sourced solutions comes with intentional and unintentional vulnerabilities or weaknesses \cite{zhang2021study} \cite{verdi2020empirical}. Software developers usually reuse code from crowd-sourced or LLMs by code obfuscation \cite{huang2023our} or structurally changing \cite{ragkhitwetsagul2019toxic} the code but keeping the functionality intact. As a result, if the original code is malicious, the developer is essentially spreading vulnerability \cite{sharif2008impeding} \cite{o2011obfuscation} in the form of  metamorphic code \cite{borello2008code}. Consequently this makes it difficult for antivirus to detect malware especially in linux environments \cite{de2021mmale} and operating systems of IoT \cite{ravi2022static} devices.


% To this end, the uncontrollable use of such advancements coupled with the chaotic OSS reuse with code and/or structural modifications impairs their effectiveness and results in critical code vulnerabilities when applied to real-world tasks \cite{wu2022ai}.

% LLM can do Code obfuscation: This involves changing the appearance of the code without changing its functionality. This can make it difficult for antivirus software to detect the malware.

%Figure \ref{fig:motivation} shows us a code generated by ChatGPT to copy a string. However, this code is vulnerable since it does not check the size of the \textit{destination} variable before copying, with a potential risk of buffer overflow. A similar study \cite{sandoval2023lost} also shows a similar finding suggesting that human interaction is essential for security analysis in LLM. 

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{1.0,1.0,1.0}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\normalsize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    frame=lines,
    rulecolor=\color{black}
}

\lstset{style=mystyle}






% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.50]{figure/motivation.pdf}
%     %\vspace{-0.3cm}
%     \caption{High level view of our proposed DevSecLLM}
%     \label{fig:fig_1}
%     %\vspace{-3mm}
% \end{figure*}

\begin{figure*}[h!]
    \centering
    % \resizebox{\linewidth}{!}{
    \includegraphics[scale=0.60]{figure/S&P-motivation-v4.pdf}
    % }
    %\vspace{-0.3cm}
    \caption{\color{red}\textbf{DevSecLLM.} Potential capabilities of our proposed model exhibited by a selected list of queries (i.e., input and instruct) and answers provided by the developed model. The first three examplary represent NOTE: While for this sample example the changes are minimal, these changes represent the capability of our work\color{red}}
    \label{fig:fig_1}
    %\vspace{-3mm}
\end{figure*}


    
\begin{comment}

\begin{figure}[h]
        \centering

        
        \lstinputlisting[language=c]{code/sample.c}
   
    \caption{A vulnerable code generated by ChatGPT. The instruction given to ChatGPT in line 1 and the comment in line 9 explain the vulnerability in line 8. The vulnerability will occur when the length of \textit{destination} is less then the length of \textit{source}.}
    \label{fig:motivation}
\end{figure}

\end{comment}

%--> Humans are not trained on code

%A recent study examined the performance of ChatGPT, an LLM-based model, in generating secure code for various coding scenarios. The findings revealed that ChatGPT produced insecure code in a majority of cases, with only limited self-correction after additional prompting. Subsequently, researchers highlighted the importance of including human interaction in evaluating the security of language models like ChatGPT to address vulnerabilities and improve overall coding robustness.


%However, these code autocompletion tools are vulnerable to attacks since the code these models were trained on datasets from publicly available sources like GitHub or StackOverflow. Moreover, the outcome of these models can be manipulated by adding specially-crafted code to the training corpus (data poisoning) during fine-tuning, which can influence its suggestions for attacker-chosen contexts \cite{schuster2021you}. In addition to that, \cite{pearce2022examining} and \cite{asare2022github} code generation models like Codex \cite{chen2021evaluating} generate vulnerabilities that were seen during training.



% \red{Importance of training the developers with vuln (Programmers are responsible for vuln- if they not expert, cant understand if llm generated code are sueucre or not)- General Description}

\textbf{Lack of Proper Security Support and Training for Software Developers.}
Software security plays a crucial role in ensuring the resilience of programs against various attacks. However, it is important to acknowledge the challenges that developers face as they are often seen as "the weakest link in the chain" when it comes to security \cite{green2016developers}. Developers bear the responsibility of making final decisions on which code goes into production. Recent research highlights the need for comprehensive security support and training for software developers to effectively address these issues \cite{green2016developers, acar2016you}. One study conducted by Assal et al. \cite{assal2019think} specifically examined the human factor in source code security. The survey shed light on the inadequate interaction between software developers and security practices. Similarly, Hermann et al. \cite{weir2020needs} conducted a survey revealing that less than a quarter of 335 successful mobile application developers had access to security experts. This alarming statistic is concerning considering the vast number of publicly available applications. It underscores the urgent need for more organized support from institutions to guide developers away from insecure coding practices. Overall, the existing approaches in software security face limitations due to the significant role of developers in the decision-making process and the need for better support and training. Addressing these issues is crucial to enhance the overall security posture in software development.



% As a result, the community has started focusing on developers whose security issues could be magnified across multiple applications \cite{acar2016you}.s


% \red{deficit with current vuln tools-- Programmers has to be in charge (Customized desc. on vul. code)}
\textbf{Deficit with Current Vulnerability Tools.}
Most deep learning-based vulnerability analyzing systems \cite{zhou2019devign}, \cite{islam2023unbiased}, \cite{chakraborty2021deep}, \cite{inproceedings} only provide information on the existence, classification, and localization of vulnerability. While sometimes automatic repair of vulnerability might be available \cite{fu2022vulrepair} \cite{pearce2022examining}, in practice, repairing a vulnerability is application and context-dependent and requires further work. Therefore, the automated repair still needs to be more reliable and far from perfect \cite{fu2022vulrepair} primarily due to the repair tool having less contextual knowledge about the entire code repository. MITRE generalizes many vulnerabilities \cite{cwe} into different categories, allowing the developer to solve vulnerabilities with categorized information. These vulnerabilities follow a generic procedure to be fixed, which needs to be checked and revised in detail by developers. However, to understand and fix vulnerabilities, a developer still has to look through a considerable amount of code and documentation to understand, categorize and fix the existing vulnerability, which takes much time and effort\cite{muegge2018time}.

%Moreover, repair is still an unreliable and far from perfect \cite{fu2022vulrepair} primarily due to the repair tool has less contextual knowledge about the entire code repository.



%Recent LLM-based tools like CodeT5 \cite{wang2021codet5}, CodeGen \cite{nijkamp2022codegen}, and CodeGeex \cite{zheng2023codegeex} perform exceptionally on code generation, code translation, and code summarization tasks performs relatively. However, the programs generated by these models come with security concerns. While these applications bring tremendous speed to the development process, they have security issues.

%. Therefore, developers must learn to write clean code by identifying and fixing these vulnerabilities. Moreover, learning to write clean code has several steps, especially for new developers. Initially, the developer needs to know what type of vulnerability exists in the code and its explanation with sufficient examples to fix it. However, to understand and fix vulnerabilities, a developer has to look through a considerable amount of code and documentation to categorize and fix the existing vulnerability, which takes much time \cite{muegge2018time}.


%In order to reduce the time and effort to analyze vulnerability, large language models like ChatGPT have started to show promising results in generating code for developers. The recent development of source code generative models like CodeT5 \cite{wang2021codet5}, CodeGen \cite{nijkamp2022codegen}, CodeGeex \cite{} performs exceptionally on code generation, code translation, and code summarization tasks performs relatively. However, the programs generated by these models come with security concerns. Figure \ref{} shows the example of a program to copy string-generated ChatGPT. However, this program can cause security issues leading to a buffer overflow of the \textit{destination} variable. Hence these models are very unreliable in understanding the security concerns of source code.


%CWE \cite{cwe} and NIST \cite{nist} provide the developers with a good view of the vulnerability landscape. But their documentation is very extensive and time-consuming to use efficiently during the software development phase. Moreover, to the best of our knowledge, no other dataset exists that can effectively train a developer with security concerns to provide a way to fix these. Some datasets like Devign \cite{zhou2019devign}, ReVeal \cite{chakraborty2021deep}, D2A \cite{zheng2021d2a} exists but are application specific. Furthermore, they do not provide any information to train a new software developer in analyzing vulnerability. Moreover, a generic communication-based system still does not exist that can provide users with quick and efficient training on vulnerability and provide a means to fix it.



%Therefore, in order to educate developers about security and provide them a secure AI-assisted tool for vulnerability repair and description generation, we propose \textbf{Some Catchy Name}, a tool for analyzing source code with security issues. We use a large language model CodeGen2 \cite{} to fine-tune for security analyzing purposes. Moreover, since this model has trained on the prompt-based dataset, we create a massive dataset containing prompts related to security and source code vulnerabilities with an appropriate English response for each prompt. Furthermore, we provide a reinforcement learning from human feedback technique to provide code-specific description which reasons why the code is vulnerable.  Our contributions are as follows: 

%%%%%%%%%%%%%%%%%
% \red{Final Paragraph: Solution}
\textbf{Our Approach.}
To address the critical need for security education among developers and offer a reliable AI-assisted solution for vulnerability repair and description generation, we propose \texttt{DevSecLLM} to identify obfuscated vulnerable code and repair them and provide a customized description. Figure \ref{fig:fig_1} shows a high-level overview of our system. Our system leverages the power of CodeGen2 \cite{nijkamp2023codegen2}, a large language model designed and fine-tuned specifically for code security analysis to identify and repair vulnerable code. To facilitate developers with a comprehensive security analysis, we curate an extensive dataset encompassing diverse prompts tailored to security concerns of source code vulnerabilities. In order to protect developers against obfuscated code, we carefully curated duplicated vulnerable to make our system more robust against attacks. In addition to vulnerability repair, we also provide a customized description using Reinforcement Learning from Human Feedback (RLHF) \cite{NIPS2017_d5e2c0ad} of the vulnerable code containing a textual description of the vulnerability of the code with its CWE category. By incorporating human feedback, we enhance the interpretability and contextual understanding of the generated descriptions.


%In addition to vulnerability detection, we propose reinforcement learning from human feedback that enables our system to generate code-specific descriptions that provide a detailed rationale for the identified vulnerabilities based on their classification. By incorporating human feedback, we enhance the interpretability and contextual understanding of the generated descriptions.

In summary, the contributions of this paper are:
\begin{itemize}
    \item We introduce a state-of-the-art AI-assisted tool designed to identify obfuscated vulnerable code and repair them with a customized description generation suited for developers with limited security knowledge. Our system leverages Reinforcement Learning from human feedback (RLHF) to enhance its capabilities and effectiveness. Initially our system determines if the function is vulnerable or not, and if the function is vulnerable, it generates the repaired code with a customized description of the code.
    

    \item To support our tool's development and protect developers against metamorphic or obfuscated code, we have compiled and released a comprehensive instruction-based vulnerability dataset. Our dataset is specifically tailored to the C/C++ programming language, emphasizing its significance in terms of security vulnerabilities. The dataset contains detailed instructions for localizing, repairing, and describing vulnerabilities, facilitating precise analysis and remediation. 
    
    
    \item Our research also includes a quantitative analysis of the results obtained from our generative tool. These models exhibit zero-shot learning capabilities, demonstrating their adaptability and robustness in vulnerability analysis with a proper ablation study. Additionally, we provide a real-world use case of our system through analyzing source code for IoT device operating system.
    
 


\end{itemize}


Combining the comprehensive instruction-based vulnerability dataset, RLHF techniques, and extensive quantitative and qualitative results analysis, our research offers a cutting-edge solution for vulnerability localization, repaired code generation, and customized description. The aim is to empower developers, particularly those with limited security knowledge, to produce code that is more resilient to attacks and minimize the occurrence of vulnerabilities.


%The organization of the remainder of this paper is outlined as follows: In Section II, we dive deep into the relevant literature and previous studies. Then we delve into the relevant literature and previous studies in Section III. Section IV outlines our preliminary work on vulnerability exploitation, setting the groundwork for the subsequent sections. Our innovative methodology is thoroughly discussed in Section V. Section VI then provides an in-depth exposition of our experimental design and results, along with a comprehensive discussion of the findings. We further substantiate our findings with an ablation study, detailed in Section VII. We conclude our work, summarizing our contributions and discussing potential future directions in Section VIII.



The paper's subsequent sections are organized as follows: In Section 2, we conduct an extensive review of pertinent literature and prior research studies. Section 3 presents an in-depth examination of preliminaries, encompassing the threat model and problem formulation. Our proposed methodology is rigorously expounded in Section 4. The details of our dataset are elaborated upon in Section 5. Subsequently, Section 6 offers a comprehensive discussion of our experimental design and results and a thorough analysis of the findings. We present an ablation study in Section 7 to substantiate our conclusions further. Finally, in Section 8, we conclude our work by summarizing our contributions and outlining potential avenues for future research with an appendix at the end.


%%%%%%%%%%%%%   Original Table 2 %%%%%%%%%%%%%%%%



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[b]
\caption{BLEU and Rouge-L score on our dataset with models trained on code. We use LLMs with multiple parameters to compare our work.}
\label{tab:tab2}
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
\textbf{Dataset}              & \textbf{Model}                 & \textbf{Parameter} & \textbf{BLEU}   & \textbf{Rouge-L} \\ \midrule
\multirow{8}{*}{InstructVul} & StarCoder                      & 1.1B               & 0.17            & 0.13             \\ \cmidrule(l){2-5} 
                              & \multirow{2}{*}{CodeT5}        & 2B                 & 0.64            & 0.71             \\
                              &                                & 6B                 & 0.73            & 0.79             \\ \cmidrule(l){2-5} 
                              & \multirow{2}{*}{CodeGen-Multi} & 2B                 & 0.54            & 0.57             \\
                              &                                & 6.7                & 0.80            & 0.98             \\ \cmidrule(l){2-5} 
                              & \multirow{2}{*}{Codegen2}      & 1B                 & 0.42            & 0.31             \\
                              &                                & 3.7B               & 0.74            & 0.91             \\ \cmidrule(l){2-5} 
                              & \textbf{CodeGen2 (Ours)}             & 7B                 & \textbf{0.82} & \textbf{0.98}    \\ %\cmidrule(l){2-5} 
                              \bottomrule
\end{tabular}
\end{table}

